The MAGPI Survey: the kinematic morphology-density relation (or lack thereof) and the Hubble sequence at $z\sim0.3$

This work presents visual morphological and dynamical classifications for 637 spatially resolved galaxies, most of which are at intermediate redshift ($z\sim0.3$), in the Middle-Ages Galaxy Properties with Integral field spectroscopy (MAGPI) Survey. For each galaxy, we obtain a minimum of 11 independent visual classifications by knowledgeable classifiers. We use an extension of the standard Dawid-Skene bayesian model introducing classifier-specific confidence parameters and galaxy-specific difficulty parameters to quantify classifier confidence and infer reliable statistical confidence estimates. Selecting sub-samples of 86 bright ($r<20$ mag) high-confidence ($>0.98$) morphological classifications at redshifts ($0.2 \le z \le0.4$), we confirm the full range of morphological types is represented in MAGPI as intended in the survey design. Similarly, with a sub-sample of 82 bright high-confidence stellar kinematic classifications, we find that the rotating and non-rotating galaxies seen at low redshift are already in place at intermediate redshifts. We \textit{do not} find evidence that the kinematic morphology-density relation seen at $z\sim0$ is established at $z\sim0.3$. We suggest that galaxies without obvious stellar rotation are dynamically pre-processed sometime before $z\sim0.3$ within lower mass groups before joining denser environments.

==> Figures/table2.tex <==
\begin{tabular}{| l  c  c|}
\hline
\textbf{Category} & \textbf{$N$} & \textbf{\textit{f}}\\
(1) & (2) & (3)\\
\hline\hline
$r<20$ mag (bright sample) & 98 & 1\\
\hline
\textit{Morphology} &&\\
\hline
$P_{\mu_{\rm Morph}} > 0.98$ & 39 & $39/98=0.4$ \\
$\mu_{\rm Morph} =$ E & 6 & $6/39=0.15$ \\
$\mu_{\rm Morph} =$ S0 & 9 & $9/39=0.23$ \\
$\mu_{\rm Morph} =$ Sp & 19 & $19/39=0.49$ \\
$\mu_{\rm Morph} =$ Irr & 0 & $0/39=0$ \\
$\mu_{\rm Morph} =$ Mer & 5 & $5/39=0.13$ \\
$\mu_{\rm Morph} =$ IDK & 0 & $0/39=0$ \\
\hline
\textit{Obvious rotation} &&\\
\hline
$P_{\mu_{\rm StellOR}} > 0.98$ & 76 & $76/98=0.78$ \\
$\mu_{\rm StellOR} =$ OR & 66 & $66/76=0.87$ \\
$\mu_{\rm StellOR} =$ NOR & 10 & $10/76=0.13$ \\
$\mu_{\rm StellOR} =$ IDK & 0 & $0/76=0$ \\
\hline
$P_{\mu_{\rm GasOR}} > 0.98$ & 64 & $64/98=0.65$ \\
$\mu_{\rm GasOR} =$ OR & 42 & $42/64=0.66$ \\
$\mu_{\rm GasOR} =$ NOR & 5 & $5/64=0.078$ \\
$\mu_{\rm GasOR} =$ IDK & 17 & $17/64=0.27$ \\
\hline
($P_{\mu_{\rm StellOR}} > 0.98$) \& ($P_{\mu_{\rm GasOR}} > 0.98$) & 62 & $62/98=0.63$ \\
($\mu_{\rm StellOR} = $ OR) \& ($\mu_{\rm GasOR} = $ OR) & 39 & $39/62=0.63$ \\
($\mu{\rm StellOR} = $ OR) \& ($\mu_{\rm GasOR} = $ NOR) & 3 & $3/62=0.048$ \\
($\mu_{\rm StellOR} = $ NOR) \& ($\mu_{\rm GasOR} = $ OR) & 2 & $2/62=0.032$ \\
($\mu_{\rm StellOR} = $ NOR) \& ($\mu_{\rm GasOR} = $ NOR) & 2 & $2/62=0.032$ \\
($\mu_{\rm StellOR} = $ IDK) | ($\mu_{\rm GasOR} = $ IDK) & 16 & $16/62=0.26$ \\
\hline
\textit{Kinematic Features} &&\\
\hline
$P_{\mu_{\rm StellFeat}} > 0.98$ & 72 & $72/98=0.73$ \\
$\mu_{\rm StellFeat} = $ WOF & 67 & $67/72=0.93$ \\
$\mu_{\rm StellFeat} = $ WF & 5 & $5/72=0.069$ \\
$\mu_{\rm StellFeat} = $ IDK & 0 & $0/72=0$ \\
\hline
$P_{\mu_{\rm GasFeat}} > 0.98$ & 67 & $67/98=0.68$ \\
$\mu_{\rm GasFeat} = $ WOF & 33 & $33/67=0.49$ \\
$\mu_{\rm GasFeat} = $ WF & 5 & $5/67=0.075$ \\
$\mu_{\rm GasFeat} = $ IDK & 29 & $29/67=0.43$ \\
\hline
($P_{\mu_{\rm StellFeat}} > 0.98$) \& ($P_{\mu_{\rm GasFeat}} > 0.98$)& 62 & $62/98=0.63$ \\
($\mu_{\rm StellFeat} = $ WF) \& ($\mu_{\rm GasFeat} = $ WF) &2 & $2/62=0.032$ \\
($\mu_{\rm StellFeat} = $ IDK) | ($\mu_{\rm GasFeat} = $ IDK) & 25 & $25/62=0.4$ \\
\hline
\end{tabular}

